Language Imbalance Driven Rewarding for Multilingual Self-improving

Large Language Models (LLMs) have achieved state-of-the-art performance across numerous tasks. However, these advancements have predominantly benefited "first-class" languages such as English and Chinese, leaving many other languages underrepresented. This imbalance, while limiting broader applications, generates a natural preference ranking between languages, offering an opportunity to bootstrap the multilingual capabilities of LLM in a self-improving manner. Thus, we propose $\textit{Language Imbalance Driven Rewarding}$, where the inherent imbalance between dominant and non-dominant languages within LLMs is leveraged as a reward signal. Iterative DPO training demonstrates that this approach not only enhances LLM performance in non-dominant languages but also improves the dominant language's capacity, thereby yielding an iterative reward signal. Fine-tuning Meta-Llama-3-8B-Instruct over two iterations of this approach results in continuous improvements in multilingual performance across instruction-following and arithmetic reasoning tasks, evidenced by an average improvement of 7.46% win rate on the X-AlpacaEval leaderboard and 13.9% accuracy on the MGSM benchmark. This work serves as an initial exploration, paving the way for multilingual self-improvement of LLMs. The code is available at https://github.com/ZNLP/Language-Imbalance-Driven-Rewarding

==> tabs/experiments_1_gsm8k_results.tex <==
\begin{table}[htbp]

\renewcommand\arraystretch{1.1}

\scriptsize

\setlength{\tabcolsep}{0.35mm}
\caption{\label{tab:results_on_mgsm_benchmark} Model Performances on MGSM benchmark.}

\begin{center}
\begin{tabular}{l|lc|lc|lc|lc|lc}
 
\toprule[1.2pt]
 
\multirow{3}{*}{\textbf{In Domain}} & \multicolumn{2}{c}{\textbf{en}} & \multicolumn{2}{c}{\textbf{es}} & \multicolumn{2}{c}{\textbf{ru}} & \multicolumn{2}{c}{\textbf{de}} & \multicolumn{2}{c}{\textbf{fr}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \noalign{\smallskip}

& \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} \\

\midrule[0.8pt]

$\text{Llama3-8B-Instruct}$
& 0.7 & 0 & 0.456 & 0.012 & 0.488 & 0.076 & 0.468 & 0.016 & 0.464 & 0.016\\

% \rowcolor{lightgray}
$+\text{MDPO}$
& 0.704 \textsubscript{\color{red}{+0.4\%}} & 0 & 0.544 \textsubscript{\color{red}{+8.8\%}} & 0 & 0.604 \textsubscript{\color{red}{+11.6\%}} & 0.004 & 0.52 \textsubscript{\color{red}{+5.2\%}} & 0 & 0.496 \textsubscript{\color{red}{+3.2\%}}& 0\\

\midrule[0.4pt]

$\text{Qwen2-7B-Instruct}$
&0.804 & 0 & 0.556 & 0.004 & 0.548 & 0.008 & 0.46 & 0.004 & 0.64 & 0.008\\

% \rowcolor{lightgray}
$+\text{MDPO}$
&0.808 \textsubscript{\color{red}{+0.4\%}} & 0 & 0.704 \textsubscript{\color{red}{+14.8\%}} & 0 & 0.7 \textsubscript{\color{red}{+15.2\%}} & 0.008 & 0.612 \textsubscript{\color{red}{+15.2\%}} & 0.004 & 0.668 \textsubscript{\color{red}{+2.8\%}} & 0\\


\midrule[0.8pt]

\multirow{3}{*}{\textbf{Out of Domain}} & \multicolumn{2}{c}{\textbf{ja}} & \multicolumn{2}{c}{\textbf{te}} & \multicolumn{2}{c}{\textbf{th}} & \multicolumn{2}{c}{\textbf{zh}} & \multicolumn{2}{c}{\textbf{bn}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \noalign{\smallskip}

& \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)}\\

\midrule[0.8pt]

$\text{Llama3-8B-Instruct}$
&0.284 &	0.28 & 0.224 & 0.012 & 0.324 & 0.124 & 0.464 & 0.336 & 0.328 & 0.024 \\

% \rowcolor{lightgray}
$+\text{MDPO}$
 & 0.328 \textsubscript{\color{red}{+4.4\%}} &	0.26 & 0.264 \textsubscript{\color{red}{+4\%}}& 0.004 & 0.396\textsubscript{\color{red}{+7.2\%}} & 0.04 & 0.48\textsubscript{\color{red}{+1.6\%}} & 0.176 & 0.448\textsubscript{\color{red}{+12\%}} & 0.004 \\


\midrule[0.4pt]

$\text{Qwen2-7B-Instruct}$
& 0.404 & 0 & 0.112 & 0 & 0.344 & 0.02 & 0.692 & 0.04 & 0.328 & 0 \\

% \rowcolor{lightgray}
$+\text{MDPO}$
&0.584 \textsubscript{\color{red}{+18\%}} & 0 & 0.168 \textsubscript{\color{red}{+5.6\%}} & 0 & 0.548 \textsubscript{\color{red}{+20.4\%}} & 0.02 & 0.696 \textsubscript{\color{red}{+0.4\%}} & 0.04 & 0.424 \textsubscript{\color{red}{+9.6\%}} & 0\\

\bottomrule[1.2pt]
\end{tabular}
\end{center}
\end{table}

==> tabs/experiments_6_gsm8k_results_qwen2.tex <==
\begin{table}[htbp]

\renewcommand\arraystretch{1.1}

\caption{\label{tab:results_on_mgsm_benchmark_qwen2}  Model Performances on MGSM benchmark on Qwen2-7B-Instruct as base model.}
\scriptsize

\setlength{\tabcolsep}{0.4mm}

\begin{center}
\begin{tabular}{l|lc|lc|lc|lc|lc}
 
\toprule[1.2pt]

\multirow{3}{*}{\textbf{In Domain}} & \multicolumn{2}{c}{\textbf{en}} & \multicolumn{2}{c}{\textbf{es}} & \multicolumn{2}{c}{\textbf{ru}} & \multicolumn{2}{c}{\textbf{de}} & \multicolumn{2}{c}{\textbf{fr}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \noalign{\smallskip}

& \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} \\

\midrule[0.8pt]
\rowcolor{lightgray}
M0
& 0.800& 0&	0.556&	0.004	&0.548&	0.008&	0.460&	0.004&	0.640&0.008\\

% \rowcolor{lightgray}
$\text{M1}$
& 0.804 \textsubscript{\color{red}{+0.4\%}} & 0 & 0.712 \textsubscript{\color{red}{+15.6\%}} & 0.004 & 0.708 \textsubscript{\color{red}{+16.0\%}} & 0.004 & 0.584 \textsubscript{\color{red}{+12.4\%}} & 004 & 0.676 \textsubscript{\color{red}{+3.6\%}}& 0\\

% $\text{M2}$
% & 0.720 \textsubscript{\color{red}{+2.0\%}} & 0 & 0.640 \textsubscript{\color{red}{+18.4\%}} & 0 & 0.620 \textsubscript{\color{red}{+13.2\%}} & 0.004 & 0.570 \textsubscript{\color{red}{+10.2\%}} & 0 & 0.608 \textsubscript{\color{red}{+14.4\%}}& 0\\

\midrule[0.8pt]

\multirow{3}{*}{\textbf{Out of Domain}} & \multicolumn{2}{c}{\textbf{ja}} & \multicolumn{2}{c}{\textbf{sw}} & \multicolumn{2}{c}{\textbf{th}} & \multicolumn{2}{c}{\textbf{zh}} & \multicolumn{2}{c}{\textbf{bn}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \noalign{\smallskip}

& \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)}\\

\midrule[0.8pt]
\rowcolor{lightgray}
M0
&0.404 &	0 & 0.064 & 0.016 & 0.344 & 0.020 & 0.692 & 0.040 & 0.328 & 0 \\

$\text{M1}$
 & 0.528 \textsubscript{\color{red}{+12.4\%}} &	0 & 0.068 \textsubscript{\color{red}{+0.4\%}}& 0.004 & 0.524 \textsubscript{\color{red}{+18.0\%}} & 0.044 & 0.740 \textsubscript{\color{red}{+4.8\%}} & 0.040 & 0.404 \textsubscript{\color{red}{+7.6\%}} & 0 \\

 % $\text{M2}$
 % & 0.476 \textsubscript{\color{red}{+19.2\%}} &	0.004 & 0.328 \textsubscript{\color{red}{+13.6\%}}& 0.002 & 0.536 \textsubscript{\color{red}{+21.2\%}} & 0 & 0.592 \textsubscript{\color{red}{+12.8\%}} & 0.064 & 0.472 \textsubscript{\color{red}{+14.4\%}} & 0 \\

\bottomrule[1.2pt]
\end{tabular}
\end{center}
\end{table}

==> tabs/experiments_7_gsm8k_iteration_results.tex <==
\begin{table}[htbp]

\renewcommand\arraystretch{1.1}

\caption{\label{tab:results_on_mgsm_benchmark}  Model Performances on MGSM benchmark on Qwen2-7B-Instruct as base model.}
\scriptsize

\setlength{\tabcolsep}{0.4mm}

\begin{center}
\begin{tabular}{l|lc|lc|lc|lc|lc}
 
\toprule[1.2pt]

\multirow{3}{*}{\textbf{In Domain}} & \multicolumn{2}{c}{\textbf{en}} & \multicolumn{2}{c}{\textbf{es}} & \multicolumn{2}{c}{\textbf{ru}} & \multicolumn{2}{c}{\textbf{de}} & \multicolumn{2}{c}{\textbf{fr}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \noalign{\smallskip}

& \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$)} & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} \\

\midrule[0.8pt]
\rowcolor{lightgray}
M0
& 0.800& 0&	0.556&	0.004	&0.548&	0.008&	0.460&	0.004&	0.640&0.008\\

% \rowcolor{lightgray}
$\text{M1}$
& 0.804 \textsubscript{\color{red}{+0.4\%}} & 0 & 0.712 \textsubscript{\color{red}{+15.6\%}} & 0.004 & 0.708 \textsubscript{\color{red}{+16.0\%}} & 0.004 & 0.584 \textsubscript{\color{red}{+12.4\%}} & 004 & 0.676 \textsubscript{\color{red}{+3.6\%}}& 0\\

% $\text{M2}$
% & 0.720 \textsubscript{\color{red}{+2.0\%}} & 0 & 0.640 \textsubscript{\color{red}{+18.4\%}} & 0 & 0.620 \textsubscript{\color{red}{+13.2\%}} & 0.004 & 0.570 \textsubscript{\color{red}{+10.2\%}} & 0 & 0.608 \textsubscript{\color{red}{+14.4\%}}& 0\\

\midrule[0.8pt]

\multirow{3}{*}{\textbf{Out of Domain}} & \multicolumn{2}{c}{\textbf{ja}} & \multicolumn{2}{c}{\textbf{sw}} & \multicolumn{2}{c}{\textbf{th}} & \multicolumn{2}{c}{\textbf{zh}} & \multicolumn{2}{c}{\textbf{bn}} \\

\cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \noalign{\smallskip}

& \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)} & \textbf{Acc($\uparrow$) } & \textbf{Off-tag($\downarrow$)}\\

\midrule[0.8pt]
\rowcolor{lightgray}
M0
&0.404 &	0 & 0.064 & 0.016 & 0.344 & 0.020 & 0.692 & 0.040 & 0.328 & 0 \\

$\text{M1}$
 & 0.528 \textsubscript{\color{red}{+12.4\%}} &	0 & 0.068 \textsubscript{\color{red}{+0.4\%}}& 0.004 & 0.524 \textsubscript{\color{red}{+18.0\%}} & 0.044 & 0.740 \textsubscript{\color{red}{+4.8\%}} & 0.040 & 0.404 \textsubscript{\color{red}{+7.6\%}} & 0 \\

 % $\text{M2}$
 % & 0.476 \textsubscript{\color{red}{+19.2\%}} &	0.004 & 0.328 \textsubscript{\color{red}{+13.6\%}}& 0.002 & 0.536 \textsubscript{\color{red}{+21.2\%}} & 0 & 0.592 \textsubscript{\color{red}{+12.8\%}} & 0.064 & 0.472 \textsubscript{\color{red}{+14.4\%}} & 0 \\

\bottomrule[1.2pt]
\end{tabular}
\end{center}
\end{table}
